InfoDense: Density-Aware Regional Decisive Replay for Memory-Efficient Incremental Face Forgery Detection

The rapid evolution of face forgery techniques has introduced an increasing variety of manipulations. Incremental Face Forgery Detection (IFFD), which incrementally adds new forgery data to fine-tune previously trained models, has emerged as a promising approach to handle evolving forgery threats. However, conventional replay-based IFFD methods suffer from catastrophic forgetting. Storing full historical images under limited memory often either fails to preserve subtle forgery cues or introduces domain bias, reducing the model's ability to learn intrinsic and transferable manipulation characteristics. In this paper, we propose a Density-Aware Regional Decisive replay strategy, termed InfoDense, to address these challenges. InfoDense prioritizes artifact-dense and forgery-critical regions, significantly reducing storage requirements while maintaining high-fidelity forgery evidence. We first introduce InfoDense Cut to localize decisive patches using CLIP-based embeddings. Then, InfoDense Select ranks candidate segments by combining latent-space representativeness and decisive patch counts, ensuring both diversity and information density in the replay buffer. Finally, InfoDense Fuse reconstructs unbiased training inputs by adaptively merging stored segments with current-task samples, enhancing knowledge retention and generalization. Extensive experiments on challenging incremental deepfake benchmarks demonstrate that InfoDense effectively mitigates catastrophic forgetting while improving cross-domain generalization.

==> ECCV_2026_Paper_Template/sec/doc/exp.tex <==
\section{Experimental Results}

\subsection{Experimental Settings} \label{sec:exp_set}
\subsubsection{Datasets.}
To construct a comprehensive benchmark that covers diverse domains and forgery techniques, we utilize a wide range of datasets. For classical benchmarks, we adopt FaceForensics++ (FF++)~\cite{FF++}, DeepFake Detection Challenge Preview (DFDCP)~\cite{dolhansky2020deepfake}, Celeb-DF-v2 (CDF)~\cite{li2020celeb}, DeepFake Detection (DFD)~\cite{DFD}, WildDeepfake (WDF)~\cite{zi2020wilddeepfake}, and UADFV \cite{li2018ictu}. To account for emerging generative threats, we further incorporate DiT and SDv21 from DF40~\cite{df40}, and SDv21 from DiffusionFace~\cite{diffusionface}. Although two datasets share the name SDv21, they originate from different sources. In our IFFD protocol, we use the SDv21 version from DiffusionFace~\cite{diffusionface} for training and evaluation, while the SDv21 version from DF40~\cite{df40} is reserved as a hold-out set to assess generalization ability.
% 数据集。为了构建一个涵盖不同领域和伪造技术的综合基准，我们使用了广泛的数据集。
% 对于经典基准，我们使用了 FaceForensics++ (FF++)、DFDCP、Celeb-DF-v2 (CDF)、DeepFake Detection (DFD)、WildDeepfake (WDF) 和 UADFV。
% 为了应对新兴的生成式威胁，我们引入了 DF40 数据集中的 DiT 和 SDv21，以及 DiffusionFace 数据集中的 SDv21。
% 值得注意的是，虽然有两个数据集都命名为 SDv21，但我们特指在增量学习协议中使用 DiffusionFace 版本，而 DF40 版本则作为保留数据集用于泛化性评估。

\subsubsection{Incremental Protocols.} 
We design two complementary incremental evaluation protocols to systematically assess the model’s plasticity and stability under evolving forgery threats:
% 增量协议。我们引入了两个不同的协议来评估模型在不断演变的伪造威胁下的可塑性和稳定性：
\begin{itemize}
    \item \textbf{Protocol 1:} 
    \textbf{Training:} The model is incrementally trained on the sequence \{FF++, DFDCP, CDF, SDv21 (DiffusionFace)\} in a continual learning manner. 
    \textbf{Testing:} After completing training on SDv21 (DiffusionFace), the resulting model is regarded as the final model. Forgetting is evaluated by testing this final model on the previously seen datasets (FF++, DFDCP, and CDF). \textit{Generalization} is assessed by evaluating its performance on SDv21 (DF40) as a held-out diffusion benchmark, as well as additional unseen datasets including UADFV, WDF, and DFD.

    % 协议 1：顺序为 {FF++, DFDCP, CDF, SDv21}。该协议混合了经典高质量数据集与最新的基于扩散模型的伪造数据，作为综合基准。
    
    \item \textbf{Protocol 2:} A sequence of \{DFDCP, SDv21 (DiffusionFace), DiT, CDF\}. This setting introduces diverse domain shifts and heterogeneous generation architectures, such as Diffusion Transformers used in DiT, thereby imposing a rigorous evaluation of the detector’s robustness and adaptability.
    % 协议 2：顺序为 {DFDCP, SDv21, DiT, CDF}。该设置引入了变化的域差距和生成架构（例如 DiT 中的扩散 Transformer），对检测器提出了严格的考验。
\end{itemize}


\subsubsection{Implementation Details.} 
Our method is implemented in PyTorch with the pre-trained CLIP ViT-L/14 as the backbone network. All input images are resized to $224 \times 224$ to satisfy the encoder requirements. The model is optimized using the Adam optimizer with an initial learning rate of $2\times10^{-4}$, a batch size of 8, and is trained for 5 epochs per task. All experiments are conducted on a single NVIDIA Tesla A100 GPU. For evaluation, frame-level Area Under the Curve (AUC) is deployed as the primary metric to measure detection performance. To further quantify catastrophic forgetting, we introduce a Performance Dropping rate (PD), defined as $PD = M_0 - M_N$, where $M_0$ represents the average AUC in the base session and $M_N$ represents the average AUC in the final session.
%实现细节。我们的方法基于 PyTorch 实现。我们采用预训练的 CLIP ViT-L/14 作为骨干网络。因此，所有输入图像均被调整大小为 224x224 以符合编码器的要求。模型使用 Adam 优化器进行优化，初始学习率为 2e-4。我们将批次大小设置为 8，每个任务训练 5 个 Epoch。所有实验均在 NVIDIA Tesla A100 和 GeForce RTX 3090 GPU 上进行。对于评估指标，我们报告帧级 AUC 作为检测准确性的主要指标。此外，我们定义了性能下降率 (PD) 来量化灾难性遗忘导致的绝对性能下降，计算公式为 $PD = M_0 - M_N$，其中 $M_0$ 是基础阶段（base session）的平均指标（AUC），$M_N$ 是最终阶段（final session）的平均指标。


\subsection{Comparison with Incremental Deepfake Detection Methods}

\begin{table}[htbp]
    \centering
        \caption{Performance comparison for face forgery detection based on Protocol 1. The two “Avg.” values denote the average detection AUC over the incremental datasets and the cross-dataset evaluation sets, respectively. The best are denoted in bold.}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{l|c|ccc|cc|cccc|c}
            \toprule
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{Venue}} & 
\multicolumn{5}{c|}{\textbf{Incremental Dataset}} & 
\multicolumn{5}{c}{\textbf{Cross-dataset}} \\

\cmidrule(lr){3-7}\cmidrule(lr){8-12}

 &  & 
\textbf{FF++} & \textbf{DFDCP} & \textbf{CDF} & \textbf{PD $\downarrow$} & \textbf{Avg.} & \textbf{SDv21} & \textbf{UADFV} & \textbf{WDF} & \textbf{DFD} & 
\textbf{Avg.} \\
            \midrule
            L-Bound & -- & 64.51 & 61.10 & 83.42 & 11.91 & 69.67 & 43.36 & 88.31 & 51.90 & 63.87 & 61.86 \\ \midrule
 LwF~\cite{li2017learning}& TPAMI' 17 & 65.32& 71.48& 76.91& 10.86& 71.24& 50.12& 87.45& 74.38& 69.24&70.30\\
 iCaRL~\cite{rebuffi2017icarl} & CVPR' 17 & 62.75& 74.36& 85.92& 10.91& 74.34& 58.47& 86.02& 60.73& 74.88&70.03\\
 DER~\cite{yan2021dynamically} & CVPR' 21 & 64.03& 79.77& 94.68& 7.35& 79.49& 66.91& 85.10& 65.89& 80.56&74.62\\
 CoReD~\cite{kim2021cored} & MM' 21 & 66.84& 82.15& 91.37& 6.92& 80.12& 72.84& 84.92& 68.77& 85.34&77.97\\
DFIL~\cite{pan2023dfil} & MM' 23 & 77.66 & 86.48 & 95.45 & 6.48 & 86.53 & 76.53 & 84.87 & 70.01 & 87.03 & 79.61 \\
 HDP~\cite{sun2025continual} & IJCV' 24 & 73.34& 81.96& 92.90& 6.59& 82.73& 60.08& 80.82& 72.59& 80.01&73.38\\
            SUR-LID~\cite{cheng2025stacking} & CVPR' 25 & 83.21 & 80.81 & 94.85 & 6.87 & 86.29 & 72.02 & 93.43 & 66.50 & 67.50 & 74.86 \\
 GPL~\cite{gpl}& ICCV'25& 77.92& 85.43& 91.99& 5.91& 85.11& 83.05& \textbf{95.17}& 72.12& 80.09&82.61\\ \midrule
            Ours & -- & \textbf{84.11} & \textbf{89.41} & \textbf{97.75} & \textbf{4.52} & \textbf{90.42} & \textbf{97.88} & 94.71 & \textbf{79.38} & \textbf{88.13} & \textbf{90.03} \\
            \bottomrule
        \end{tabular}%
    }
    \label{tab:comparison}
\end{table}
 
% 表格 1：协议 1 上的 SOTA 方法性能对比。
% 注意：为了简洁起见，第 4 个增量任务（来自 DiffusionFace 的 SDv21）未明确显示。
% SDv21 列指的是来自 DF40 的未见数据集。
% PD 表示平均性能下降率。
% 第一个 Avg. 代表三个历史任务的平均准确率（Pre-Avg），不包括最终阶段。

We evaluate the proposed InfoDense against state-of-the-art incremental face forgery detection methods under Protocol 1, aiming to verify its advantages in both continual learning stability and cross-domain generalization. As shown in Tab.~\ref{tab:comparison}, InfoDense achieves the lowest PD among all compared methods. This result demonstrates its strong resistance to catastrophic forgetting on previously learned datasets such as FF++, DFDCP, and Celeb-DF. Unlike existing approaches that store complete historical images and suffer from limited replay diversity, InfoDense removes task-irrelevant background regions. This design enables substantially higher replay diversity under the same memory budget. The enriched historical distribution improves stability across incremental tasks.

More importantly, InfoDense guides the model to focus on highly concentrated and decisive forgery fragments rather than entire facial regions. This encourages the learning of intrinsic and transferable forgery cues instead of dataset-specific biases. As a result, the method shows clear gains in cross-domain generalization and significantly outperforms competitors such as SUR-LID on challenging unseen datasets like WDF.

% 我们在协议 1 上将提出的 InfoDense 与最先进的增量人脸伪造检测方法进行了评估。不同于现有方法静态存储完整历史图像并受限于回放多样性，InfoDense 主动剥离了与任务无关的冗余背景，从而在完全相同的内存预算下实现了显著更高的回放多样性。这种扩展的历史分布使我们的方法在 FaceForensics++、DFDCP 和 Celeb-DF 等先前任务上实现了最低的性能下降率和卓越的稳定性。更重要的是，通过迫使网络不断重温高度集中的决定性片段而不是完整人脸，模型捕捉到了本质的、可迁移的伪造痕迹，而不是过拟合于特定数据集的域偏差。这种范式转变为未见领域带来了卓越的泛化能力，特别是在具有挑战性的野外数据集 WDF 上大幅超越了 SUR-LID 等竞争对手。

\subsection{Ablation Study on Compression Strategies}

\subsubsection{Comparison with Global Compression Baselines.}
A comparison with global compression baselines, including JPEG at different compression ratios and CIM, is presented in Tab.~\ref{tab:ablation}. Moderate global compression enables more historical samples to be stored and brings a slight performance improvement over the uncompressed baseline. However, as the compression ratio increases, subtle high-frequency artifacts that are critical for deepfake detection are progressively destroyed, resulting in significant performance degradation. This phenomenon highlights the intrinsic limitation of global lossy compression, which reduces memory usage at the expense of indiscriminately damaging essential forgery traces. In contrast, InfoDense avoids this trade-off by adopting spatial compression rather than quality compression. Task-irrelevant background regions are removed, while the original, uncompressed pixels in information-dense areas are strictly preserved. This design maintains high-fidelity forgery cues and ensures more robust knowledge preservation under the same memory budget.

% \subsubsection{与压缩基线的比较}
% 我们首先将我们的方法与包括不同压缩比率的 JPEG 和 CIM 在内的全局压缩基线进行了评估。虽然适度的全局压缩允许存储更多历史样本，并在最初比未压缩的基线获得了性能提升，但进一步提高压缩比率不可避免地会破坏对深度伪造检测至关重要的微小高频伪影，导致严重的性能下降。这暴露了全局有损压缩的固有缺陷，即它不加区分地牺牲关键伪造痕迹的保真度来节省内存空间。形成鲜明对比的是，InfoDense 通过执行空间压缩而非质量压缩，完全规避了这一困境。通过完全丢弃与任务无关的背景，同时严格保留信息密集区域未经压缩的原始像素，我们的策略确保了核心伪造线索的高保真保留，从而实现了最稳健的知识保存。

\subsubsection{Impact of Regional Shapes and Patch Selection.}

We further analyze the influence of region shapes (Rectangular vs.\ Fan-shaped) and patch selection strategies (Random vs.\ Density-Aware). As reported in Tab.~\ref{tab:ablation}, \textbf{Cut} and \textbf{Clock} denote rectangular and fan-shaped base regions, respectively. \textbf{Mix} indicates random patch sampling, while the incorporation of $\mathbf{P_D}$ and our proposed \textbf{InfoDense} leverage decisive patch density to guide the patch selection process.

\begin{itemize}
\item \textbf{Rectangular vs.\ Fan-shaped.}
Under random patch sampling, the fan-shaped \textbf{ClockMix} consistently outperforms the rectangular \textbf{CutMix}. Facial structures and forgery artifacts often exhibit a center-symmetric spatial distribution. Fan-shaped sectors radiating from the facial center are therefore more likely to preserve critical structural and manipulation cues. In contrast, randomly sampled rectangular patches may exclude the facial center, resulting in inferior knowledge retention.

\item \textbf{Random vs.\ Density-Aware Patch Selection.}
The advantage of density-aware guidance based on decisive patches $\mathbf{P_D}$ is evident. Purely random sampling leads to a low coverage of decisive regions, reflected by the small \textbf{nSeg} values observed in both \textbf{CutMix} and \textbf{ClockMix}. When patch selection is guided by the density of $\mathbf{P_D}$, both \textbf{CutMix+$\mathbf{P_D}$} and \textbf{InfoDense} show a significant increase in information concentration. By aligning the center-symmetric fan-shaped regions with the intrinsic spatial density of forgery cues, \textbf{InfoDense} achieves a more effective balance between spatial compression and discriminative performance.
\end{itemize}

% \subsubsection{区域形状与提取引导机制的影响。}
% 我们进一步研究了区域形状（包括矩形和扇形）以及提取引导策略（包括随机裁剪和我们提出的密度感知提取）的影响。在表 2 中，Cut 和 Clock 分别表示基础的矩形和扇形区域。Mix 代表随机提取，而引入 P_D 以及我们提出的 InfoDense 则是利用决定性 Patch 的密度来主动引导提取过程。
    
    % 矩形 vs. 扇形：当比较随机提取基线时，扇形的 ClockMix 天然优于矩形的 CutMix。由于面部特征和伪造痕迹通常表现出中心对称的分布，从面部中心辐射出的扇形区域本质上能捕捉到更多关键的结构信息。相反，随机的矩形裁剪很容易完全错过关键的面部中心，导致较差的知识保留。

    
    
    % 随机 vs. 密度感知提取：利用决定性 Patch P_D 进行提取引导的必要性非常明显。仅依赖随机裁剪会导致决定性 Patch 的包含量极低，这从 CutMix 和 ClockMix 较低的 nSeg 指标中可以看出。通过引入 P_D 的密度来引导提取，CutMix+P_D 和我们的 InfoDense 在信息密度上都实现了大幅提升。最终，我们的 InfoDense 策略完美地将中心对称的扇形提取与伪造线索的内在空间密度对齐，在空间压缩和判别性能之间实现了最佳平衡。

\begin{table}[t]
    \centering
    \tiny
        \caption{Ablation Study on Compression Strategies. \textbf{nSeg} represents the task-averaged number of decisive patches contained in a single replay segment.}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{l|c|ccc|cc|cccc|c}
            \toprule
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{nSeg}} & 
\multicolumn{5}{c|}{\textbf{Incremental Dataset}} & 
\multicolumn{5}{c}{\textbf{Cross-dataset}} \\

\cmidrule(lr){3-7}\cmidrule(lr){8-12}

 &  & 
\textbf{FF++} & \textbf{DFDCP} & \textbf{CDF} & \textbf{PD $\downarrow$} & \textbf{Avg.} & \textbf{SDv21} & \textbf{UADFV} & \textbf{WDF} & \textbf{DFD} & 
\textbf{Avg.} \\
            \midrule
            Base(DFIL) & -- & 77.66 & 86.48 & 95.45 & 6.48 & 86.53 & 43.36 & 88.31 & 51.90 & 63.87 & 61.86 \\
            JPEG (Q=50) & -- & 73.22 & 89.11 & 94.34 & 4.84 & 85.55 & 71.99 & 88.24 & 70.54 & 82.73 & 78.37 \\
            JPEG (Q=95) & -- & 79.26 & 84.03 & 91.45 & 5.16 & 84.91 & 79.29 & 94.22 & 79.28 & 91.40 & 86.04 \\
            CIM\cite{luo2023class} & -- & 83.12 & 87.18 & 94.94 & 4.97 & 88.41 & 89.04 & 94.60 & 71.82 & 82.20 & 84.41 \\
            CutMix & 3.86 & 72.34 & 76.24 & 90.38 & 6.72 & 79.65 & 57.14 & 93.52 & 75.21 & 73.98 & 74.96 \\
            CutMix+$\mathbf{P}_\text{D}$ & 7.52 & 79.83 & 83.13 & 93.94 & 6.31 & 85.63 & 62.70 & 87.29 & 68.31 & 84.46 & 75.69 \\
            ClockMix & 3.34 & 78.12 & 87.00 & 93.85 & 6.01 & 86.32 & 83.40 & 84.56 & 73.78 & 81.20 & 80.58 \\
            Ours & 8.31 & 84.11 & 89.41 & 97.75 & 4.52 & 90.42 & 97.88 & 94.71 & 79.38 & 88.13 & 90.03 \\
            \bottomrule
        \end{tabular}%
    }
    \label{tab:ablation}
\end{table}

% 表格 2：压缩策略消融实验。
% 注意：为了简洁起见，第 4 个增量任务未明确显示。
% SDv21 列指的是来自 DF40 的未见数据集。
% PD 表示平均性能下降率。
% 第一个 Avg. 代表三个历史任务的平均准确率（Pre-Avg）。
% Cvg. (覆盖率) 表示回放区域中包含的前 10 个关键 Patch (top-10 decisive patches) 的平均数量，该指标是在 FF++ 数据集上计算得出的。

\subsection{Ablation on Selection and Fusion Strategies}

\subsubsection{Effectiveness of Selection Strategy.}
As shown in Tab.~\ref{tab:selection_strategy}, the effectiveness of the InfoDense selection strategy is evaluated against Random, Center, and Center+Hard baseline sampling methods. For the Center strategy, the weight of the decisive patch count is set to zero and selection relies solely on the latent-space centroid distance to maintain distribution representativeness. Although prioritizing central samples or decision-boundary proximal hard samples brings slight improvements over random selection, these strategies construct the replay buffer without explicitly verifying whether the sampled fragments contain authentic forgery artifacts. As a result, they often fail to preserve sufficient task-relevant cues. In contrast, InfoDense dynamically integrates centroid distance with the explicit count of decisive patches. This design filters out redundant background regions and ensures that the replay buffer is densely populated with artifact-rich fragments. The dual-metric selection mechanism substantially mitigates catastrophic forgetting and provides high-quality replay data, thus enabling stronger generalization across diverse unseen domains.

% \subsubsection{选择策略的有效性}
% 为了评估 InfoDense 选择策略的有效性，我们将它与 Random、Center 和 Center+Hard 基线采样方法进行了比较。Center 策略作为一个关键的消融实验，实际上是将决定性 Patch 计数的权重完全设为零，仅依赖潜在空间的质心距离来保证分布的代表性。虽然优先选择中心或靠近决策边界的困难样本比随机选择有微小的提升，但这些策略在构建回放缓冲区时，盲目地忽略了裁剪片段中是否物理上存在伪造伪影。因此，它们无法捕获足够的任务相关线索。通过将质心距离与决定性 Patch 的显式计数动态结合，我们的 InfoDense 策略刻意过滤掉了冗余背景，并确保回放缓冲区内密集充斥着核心的伪造证据。这种双指标选择不仅大幅减少了灾难性遗忘，还提供了高质量、富含伪影的演练数据，从而解锁了在各种未见领域上的强大泛化能力。

\begin{table}[t]
    \centering
    \tiny
    \caption{Ablation study on regional selection strategies. \textbf{nSeg}  represents the task-averaged number of decisive patches contained in a single replay segment.}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{l|c|ccc|cc|cccc|c}
            \toprule
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{nSeg}} & 
\multicolumn{5}{c|}{\textbf{Incremental Dataset}} & 
\multicolumn{5}{c}{\textbf{Cross-dataset}} \\

\cmidrule(lr){3-7}\cmidrule(lr){8-12}

 &  & 
\textbf{FF++} & \textbf{DFDCP} & \textbf{CDF} & \textbf{PD $\downarrow$} & \textbf{Avg.} & \textbf{SDv21} & \textbf{UADFV} & \textbf{WDF} & \textbf{DFD} & 
\textbf{Avg.} \\
            \midrule
            Random      & 3.34 & 79.02 & 78.51 & 92.23 & 6.58 & 83.25 & 83.40 & 84.56 & 73.78 & 81.20 & 80.58 \\
            Center      & 6.46 & 80.26 & 84.20 & 94.93 & 5.80 & 86.46 & 84.87 & 89.32 & 72.86 & 76.58 & 80.90 \\
            Center+Hard & 6.64 & 80.46 & 83.15 & 96.11 & 5.56 & 86.57 & 79.00 & 83.74 & 70.48 & 83.80 & 79.25 \\
            Ours        & 8.31 & 84.11 & 89.41 & 97.75 & 4.52 & 90.42 & 97.88 & 94.71 & 79.38 & 88.13 & 90.03 \\
            \bottomrule
        \end{tabular}%
    }
    \label{tab:selection_strategy}
\end{table}

\subsubsection{Effectiveness of Fusion Strategy.}
To validate the effectiveness of the InfoFuse strategy, we compare it with two simplified variants: isolated historical self-fusion ($({t-1})\&({t-1})$) and inter-task-only fusion ($(t-1)\&(t)$). As shown in Tab.~\ref{tab:fusion_strategy}, isolated self-fusion leads to severe catastrophic forgetting. This is because reconstructing replay samples solely from historical data introduces a pronounced domain gap between fused replay samples and pristine current-task images, thereby amplifying task bias. Inter-task-only fusion, which pastes historical segments onto current images, partially alleviates this domain discrepancy. However, its generalization performance remains sub-optimal. Without intra-task mixing applied to current data, the model can exploit artificial fusion boundaries as shortcut cues to distinguish task identities rather than learning intrinsic forgery patterns. In contrast, our complete InfoFuse strategy jointly performs inter-task and intra-task mixing. By exposing the deep network to fusion boundaries across all data distributions, InfoFuse reduces sensitivity to boundary artifacts and encourages the model to focus on genuine forgery traces. As evidenced in Tab.~\ref{tab:fusion_strategy}, this unified design achieves stronger knowledge retention and improved generalization performance.

% \subsubsection{融合策略的有效性}
% 为了验证我们的 InfoFuse 策略，我们将它与孤立的历史自我融合（$t-1_{t-1}$）和仅跨任务融合（$t-1_t$）进行了比较。孤立的自我融合会导致严重的灾难性遗忘，因为它在重建的回放样本和原始当前数据之间产生了明显的领域鸿沟，严重诱发了任务偏差。相反，直接将历史片段粘贴到当前图像上弥合了这一鸿沟，但泛化能力依然次优。在没有对当前数据应用任务内混合的情况下，网络极易利用人为的融合边界作为区分任务的虚假捷径。我们全面的 InfoFuse 通过同时执行跨任务和任务内混合解决了这一缺陷。通过让网络在所有数据分布中暴露于融合边界，InfoFuse 迫使模型对拼接伪影脱敏并纯粹关注内在伪造线索，从而确保了稳健的知识保留和强大的泛化能力。

\begin{table}[t]
    \centering
    \tiny
    \caption{Ablation study on inter-task and intra-task fusion strategies. $({t-1})\&({t-1})$ and $(t-1)\&(t)$ denote isolated historical self-fusion and inter-task fusion without intra-task mixing, respectively.}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{l|ccc|cc|cccc|c}
            \toprule
\multirow{2}{*}{\textbf{Method}} & 

\multicolumn{5}{c|}{\textbf{Incremental Dataset}} & 
\multicolumn{5}{c}{\textbf{Cross-dataset}} \\

\cmidrule(lr){2-6}\cmidrule(lr){7-11}

 &  
\textbf{FF++} & \textbf{DFDCP} & \textbf{CDF} & \textbf{PD $\downarrow$} & \textbf{Avg.} & \textbf{SDv21} & \textbf{UADFV} & \textbf{WDF} & \textbf{DFD} & 
\textbf{Avg.} \\
            \midrule
            $({t-1})\&({t-1})$     & 63.75 & 61.27 & 80.11 & 12.23 & 68.37 & 63.29 & 86.65 & 59.88 & 66.63 & 69.11 \\
            $(t-1)\&(t)$     & 79.23 & 89.75 & 94.72 & 4.91  & 87.90 & 72.74 & 96.19 & 67.62 & 80.74 & 79.32 \\
            Ours  & 84.11 & 89.41 & 97.75 & 4.52  & 90.42 & 97.88 & 94.71 & 79.38 & 88.13 & 90.03 \\
            \bottomrule
        \end{tabular}%
    }
    \label{tab:fusion_strategy}
\end{table}

\subsection{Analysis of Storage Efficiency and Redundancy}

We conduct extensive experiments to analyze the storage efficiency of our method and verify the intrinsic redundancy hypothesis in face forgery data from two perspectives: the storage-performance trade-off and empirical redundancy limits.

% \subsection{存储效率与冗余性分析}
% 我们从存储-性能权衡和经验冗余极限两个角度，进行了广泛的实验来分析我们方法的存储效率，并验证人脸伪造数据中的内在冗余假设。

\subsubsection{Performance Evaluation on Storage Efficiency.}
In practical deployment, maximizing detection accuracy under limited storage is a critical Pareto optimization problem. We evaluate this trade-off by comparing InfoDense with the full-image replay baseline DFIL under different compression ratios. As shown in Fig.~\ref{fig:storage}, InfoDense consistently achieves a clearly superior Pareto frontier. Under the same memory budget, allocating storage to a larger number of compressed, information-dense fragments significantly outperforms storing fewer complete images. For example, retaining fragments at one quarter of the original size yields higher detection accuracy than the baseline that stores the same number of intact images, while consuming only a fraction of the memory. These results demonstrate that density-aware selection effectively removes redundant background content and allows the replay buffer to preserve a much richer diversity of critical forgery cues within strict storage constraints.

% \subsubsection{存储效率的性能评估}
% 在实际部署中，以最小的存储消耗实现最大的检测准确率是一个关键的 Pareto 优化问题。我们通过比较 InfoDense 策略在不同压缩比下与全图回放基线 DFIL 的表现来评估这一权衡。如图~\ref{fig:storage} 所示，我们的方法始终建立了一个极具优势的 Pareto 前沿。具体而言，在完全相同的内存预算下，将存储空间分配给大量压缩的、信息密集的片段，大幅优于存储少量完整图像。例如，存储大量压缩至原大小四分之一的片段，其准确率甚至高于存储相同数量全图的基线，同时仅消耗了一小部分总内存。这证明了我们的密度感知选择成功过滤掉了冗余背景，使模型能够在严格的存储限制内，存档显著更丰富多样的关键伪造线索。

% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=1\linewidth]{ECCV_2026_Paper_Template/sec/fig/storage.pdf}
%     \caption{Storage Per Task.}
%     \label{fig:storage}
% \end{figure*}

\begin{figure}[t]
\centering
\begin{minipage}{0.6\textwidth}
  \centering
  \includegraphics[width=\linewidth]{ECCV_2026_Paper_Template/sec/fig/vit.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.38\textwidth}
  \centering
  \includegraphics[width=\linewidth]{ECCV_2026_Paper_Template/sec/fig/cnn.pdf}
\end{minipage}
\caption{Storage-performance Pareto frontier under varying replay budgets. (Left) Results evaluated on Protocol 1. (Right) Results evaluated on Protocol 2.}
% 图 4：不同回放预算下的存储-性能 Pareto 前沿。（左图）在 Protocol 1 上的评估结果。（右图）在 Protocol 2 上的评估结果。
\label{fig:storage}
\end{figure}

\subsubsection{Verification of Facial Redundancy.}
To empirically validate the inherent redundancy of face forgery data, we conduct a supplementary experiment utilizing a random fan-shaped cropping strategy on a naive CNN backbone (Fig.~\ref{fig:storage} Right). Here, we discard the strategic selection process and stochastically extract regional segments to evaluate the structural resilience of forgery cues. Strikingly, the performance curves reveal that this purely random extraction consistently outperforms the full-image baseline. This counter-intuitive superiority confirms our core motivation that forgery traces are highly redundant and center-symmetric. It provides strong empirical evidence that archiving the entire face fundamentally limits the potential diversity of the replay buffer, whereas even stochastically sampled partial regions intrinsically encapsulate sufficient discriminative information to drive a more robust incremental replay.

% \subsubsection{人脸冗余性的验证}
% 为了从经验上验证人脸伪造数据的内在冗余性，我们在标准 CNN 骨干网络上利用随机扇形裁剪策略进行了一项补充实验。与密度感知的 InfoDense 不同，该设置完全放弃了策略性选择过程，而是随机提取局部扇形区域以评估伪造线索的结构韧性。令人惊讶的是，性能曲线显示这种纯随机提取始终优于全图基线。这种反直觉的优越性证实了我们的核心动机，即伪造痕迹是高度冗余且中心对称的。它提供了强有力的经验证据，表明存档整张人脸从根本上限制了回放缓冲区的潜在多样性，而即使是随机采样的局部区域，本质上也封装了足够的判别信息来驱动更稳健的增量演练。


\subsection{Robustness against Image Degradations}
To verify that the proposed regional decisive replay mechanism does not overfit to high-quality pristine data, we evaluate the model stability against common real-world image degradations. During the inference phase, we independently apply four types of perturbations including downsampling, saturation alteration, block-wise drop, and JPEG compression. Each degradation is configured with five progressive severity levels to comprehensively assess the performance decay trend, with average AUC as the evaluation metric. As illustrated in Fig.~\ref{fig:robustness}, our method consistently exhibits superior resilience against varying degrees of corruptions compared to the baseline. This demonstrates that by selectively replaying information-dense regions, the model avoids relying on fragile artifacts and successfully learns robust, intrinsic forgery traces.

%图像退化的鲁棒性。为了验证所提出的区域决定性回放机制没有对高质量的干净数据产生过拟合，我们评估了模型在面对现实世界中常见图像退化时的稳定性。在推理阶段，我们独立地施加了四种类型的扰动，包括下采样、饱和度改变、块状丢弃和 JPEG 压缩。每种退化均配置了五个递进的强度等级，以全面评估性能的衰减趋势。我们评估了四个标准深伪数据集的平均检测性能。如图~\ref{fig:robustness} 所示，与基线模型相比，我们的方法在面对不同程度的破坏时始终表现出更优越的抗干扰能力。这证明了通过选择性地回放信息密集的区域，模型避免了依赖脆弱的伪影，并成功学习到了能够抵御严重图像破坏的鲁棒且本质的伪造痕迹。

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{ECCV_2026_Paper_Template/sec/fig/robustness_1x4.pdf}
    \caption{Robustness evaluation against test-time common image degradations across five progressive severity levels.}
    \label{fig:robustness}

\end{figure*}


\subsection{Visualization Analysis on InfoDense Fuse}
To demonstrate that our segment fusion strategy maintains the discriminability of deepfake features without introducing seaming-induced confusion, we visualize the latent space using UMAP \cite{umap}. Fig.~\ref{fig:vis}(a) illustrates the feature distributions of original Task $t$ samples alongside intra-task self-fused samples. The fused features seamlessly align with their corresponding original real and fake clusters, proving that the fusion operation preserves the intrinsic class distributions. Fig.~\ref{fig:vis}(b) compares the original Task $t$ samples with the inter-task replay samples (Task $t-1$ segments fused onto Task $t$). The replay samples heavily overlap with their respective real and fake domains, maintaining strict class separability. This confirms that our approach successfully constructs valid replay data that retains core forgery cues, enabling effective historical knowledge accumulation without distorting the feature space.

%潜在空间可视化。为了直观地证明我们的片段融合策略在不引入边界混淆的情况下保持了伪造特征的判别力，我们使用 UMAP 对潜在特征空间进行了可视化。图~\ref{fig:vis}(a) 展示了原始任务 t 样本以及任务内自融合样本的特征分布。融合后的特征与其对应的原始真伪聚类无缝对齐，证明拼接操作保留了内在的类别分布。图~\ref{fig:vis}(b) 比较了原始任务 t 样本与跨任务回放样本（任务 t-1 片段融合到任务 t 上）。回放样本与其各自的真伪域高度重合，保持了严格的类别可分性。这证实了我们的方法成功构建了保留核心伪造线索的有效回放数据，从而在不扭曲特征空间的情况下实现了有效的历史知识积累。

\begin{figure}[h]
\centering
\begin{minipage}{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{ECCV_2026_Paper_Template/sec/fig/t.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{ECCV_2026_Paper_Template/sec/fig/t-1.pdf}
\end{minipage}
\caption{UMAP visualization of the latent space. (a) Original Task $t$ samples \textit{vs.} intra-task self-fused samples. (b) Original Task $t$ samples \textit{vs.} inter-task replay samples.}
\label{fig:vis}
\end{figure}

%图~\ref{fig:vis} 潜在空间的 UMAP 可视化。(a) 原始任务 t 样本与任务内自融合样本的特征分布。(b) 原始任务 t 样本与跨任务回放样本的特征分布。

\subsection{Privacy Quantitative Analysis}


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{ECCV_2026_Paper_Template/sec/fig/privacy.pdf}
    \caption{Quantitative Analysis of Identity Privacy Protection. The Top-1 and Top-3 recall rates indicate the probability of successfully retrieving the original identity from the stored replay samples using face recognition models (\textit{i.e.}, ArcFace and CosFace). Lower matching rate indicates lesser identity leakage.}
    % 身份隐私的定量分析。Top-1 和 Top-3 召回率表示使用最先进的人脸识别模型从存储的回放样本中成功检索出原始身份的概率。
    \label{fig:privacy}
   
\end{figure}

A critical concern in replay-based incremental learning is the potential privacy leakage associated with storing historical user data. To quantitatively evaluate the privacy preservation capability of our approach, we measure the identity retrieval recall rate of stored samples against original faces using state-of-the-art face recognition models including ArcFace \cite{deng2019arcface} and CosFace \cite{wang2018cosface}. As reported in Fig.~\ref{fig:privacy}, traditional global compression methods severely compromise user privacy, maintaining near-perfect retrieval recall even at higher compression rates. This occurs because global compression uniformly preserves the holistic facial topology essential for identity recognition. In stark contrast, InfoDense completely shatters this holistic structure by selectively isolating highly localized forgery-decisive fragments. Consequently, standard recognition networks fail to extract coherent identity embeddings, resulting in a near-zero retrieval recall. This compellingly demonstrates that InfoDense not only optimizes storage efficiency but inherently acts as a robust de-identification mechanism, making it highly suitable for privacy-sensitive practical deployments.

% 基于回放的增量学习中的一个关键问题是与存储历史用户数据相关的潜在隐私泄露风险。为了定量评估我们方法的隐私保护能力，我们使用包括 ArcFace 和 CosFace 在内的最先进人脸识别模型，测量了存储样本与原始人脸的身份检索召回率。如表~\ref{tab:privacy} 所示，传统的全局压缩方法严重损害了用户隐私，即使在较高的压缩率下也保持着近乎完美的检索召回率。这是因为全局压缩均匀地保留了对身份识别至关重要的整体面部拓扑结构。形成鲜明对比的是，InfoDense 通过有选择地隔离高度局部的伪造决定性片段，彻底破坏了这种整体结构。因此，标准的识别网络无法提取连贯的身份嵌入，导致检索召回率接近于零。这有力地证明了 InfoDense 不仅优化了存储效率，而且本质上充当了一种稳健的脱敏机制，使其非常适合对隐私敏感的实际部署。


==> ECCV_2026_Paper_Template/sec/doc/intro.tex <==
\section{Introduction}
The rapid advancement of generative technologies has led to increasingly diverse and realistic forgery faces, posing serious threats to multimedia security and social trust. One line of research seeks to address this challenge by training forgery detection models with strong generalization ability under limited data conditions, so as to improve robustness to unseen forgeries. However, generalization-oriented approaches \cite{sun2022dual,cao2022end,huang2023implicit,yan2024transcending,cheng2024can,cheng2025ed} can only partially handle unknown forgery patterns and still struggle to cope with the continuous evolution of forgery techniques. To this end, incremental forgery detection has recently attracted growing attention, aiming to progressively learn new forgery types while maintaining reliable detection performance on previously learned ones.

Incremental forgery detection methods typically mitigate catastrophic forgetting by replaying representative samples during the learning of new data. Common strategies include central sample replay \cite{pan2023dfil}, hard sample replay \cite{pan2023dfil}, adversarial perturbation–based replay \cite{sun2025continual}, mixed prototypes \cite{tian2024dynamic}, and sparse uniform replay \cite{cheng2025stacking}. However, these replay-based approaches inevitably require storing raw historical samples, resulting in non-negligible memory overhead and potential privacy risks. Please refer to Appendix Sec.~\ref{related work} for detailed illustrations of \textbf{\textit{Related Work}}. Notably, face images exhibit strong structural regularities, such as bilateral symmetry and the spatial concentration of discriminative cues. For deepfake detection, the information required for effective replay mainly concerns identity-related features, forgery artifacts, and domain-specific patterns. These cues are typically localized and redundantly distributed across symmetric facial regions rather than uniformly over the entire face. Hence, storing the full face image may be unnecessary to preserve replay knowledge, while selectively retaining informative regions can sufficiently maintain the critical information needed to mitigate forgetting in incremental deepfake detection.


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{sec/fig/intro.pdf}
    \caption{Intuitive impression of our motivation, \textit{i.e.}, replaying infodense segment insead of replaying redundant full faces.}
    \label{fig:intro}
\end{figure}

Motivated by the above observations, we aim to design a \textbf{regional decisive replay} strategy that preserves essential forgery knowledge while significantly reducing storage cost. As shown in Fig. \ref{fig:intro}, we model and visualize the decisive attention of samples during detector training. According to the resulting attention distribution, forgery face images can be conceptually divided into \textbf{information-dense} and \textbf{information-sparse} regions. The \textbf{former} is sufficient to capture critical domain characteristics and \textbf{forgery traces}, while the \textbf{latter} mainly contains \textbf{redundant content}. Furthermore, the empirical results in Fig. \ref{fig:illustration} validate the substantial potential of compressing redundant facial information. Even when only a fraction of each image is retained, the detection performance remains highly competitive, indicating that intact facial images contain considerable redundancy for replay. Based on this insight, we preferentially retain information-dense regions during replay, \textbf{enabling effective knowledge preservation with significantly reduced memory cost}. As a result, more historical samples can be stored under the same budget, alleviating catastrophic forgetting. Meanwhile, concentrating replay on compact yet decisive regions encourages the detector to focus on intrinsic forgery cues, thereby improving generalization to unseen manipulations.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{ECCV_2026_Paper_Template/sec/fig/illustration.pdf}
    \caption{Performance impression on compressing redundant facial information. The results are obtained with Protocol 1 (see Sec.~\ref{sec:exp_set}). \textbf{n} in Compression Rate denotes $\frac{1}{\text{n}}$ segment of one intact image is used for replay. Replay Diversity is represented by the number of image samples stored in the replay set. With significantly reduced storage, two different versions of our approach achieve comparable performance against the baseline, indicating the redundancy of using intact face images as the replay samples.}
    \label{fig:illustration}
\end{figure}
In this paper, we propose a Density-Aware Regional Decisive replay strategy, termed InfoDense, for memory-efficient incremental deepfake detection. The goal is to preserve forgery-critical information under limited replay capacity. We first introduce \textbf{InfoDense Cut} to estimate the regional density of decisive forgery cues. Patch-level image tokens are extracted using a CLIP-based encoder. Each token is assigned a forgery-decisive score based on its similarity to forgery-representative text embeddings. The top-$K$ patches are selected as Decisive Patches to localize the most discriminative regions. We then perform \textbf{InfoDense Select} to rank candidate segments. The ranking is based on a weighted combination of latent-space centroid distance and decisive patch count. The top-$m$ segments are stored in the replay buffer to ensure both representativeness and information density. Finally, we apply \textbf{InfoDense Fuse} to adaptively combine stored segments with current-task samples. This process reconstructs complete training inputs and enables effective and unbiased replay. It also enriches fine-grained forgery evidence and mitigates catastrophic forgetting during incremental learning. Our contributions can be summarized as follows:
\begin{itemize}
\item By exploiting the inherent redundancy in facial information, InfoDense significantly reduces storage requirements. Under the same memory budget, it enables a multiplicative increase in replay diversity, thereby effectively alleviating catastrophic forgetting in incremental learning.
\item InfoDense distills core forgery-decisive cues and reuses them across multiple tasks, encouraging the model to capture intrinsic forgery characteristics rather than task-specific artifacts, thus improving generalization ability.
\item Since the replay buffer stores only compact decisive regions instead of complete facial images, InfoDense naturally mitigates potential privacy risks associated with data replay, making it more suitable for practical deployment.
\end{itemize}
% \textcolor{red}{Yry:There are too many lines with only a few letters or words occupying an entire line.}



==> ECCV_2026_Paper_Template/sec/doc/method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{sec/fig/pipeline.pdf}
    \caption{Overall pipeline of the proposed InfoDense. We first propose a replay cut\&select strategy to obtain informative regional replay segments. We then utilize these segments to achieve effective replay learning that mitigates catastrophic forgetting while improving diversity for generalization.}
    \label{fig:pipeline}
\end{figure*}
\section{Proposed Method}
To compress the redundant information in the facial data, thus improving the diversity and information density under the limit of the same storage consumption, we propose a unified framework termed InfoDense that can cut, select, and utilize the regional segments with dense information for replay. The overall pipeline can be found in Fig.~\ref{fig:pipeline}.
\subsection{Rational Behind Compressing Facial Information}
Facial images contain substantial structural redundancy due to the strong spatial regularity and identity consistency of human faces. A large portion of a face, including smooth skin regions such as the cheeks, forehead, and jaw area, exhibits low-frequency and homogeneous appearance that remains stable across frames, poses, and expressions. These regions primarily encode identity-related information and contribute little to forgery detection. In contrast, deepfake detectors mainly rely on subtle local inconsistencies introduced during synthesis and blending, which are typically concentrated around semantically sensitive regions such as the eyes, mouth, nose boundary, and facial contour. As a result, the majority of facial pixels provide highly correlated and repetitive signals from the perspective of the detection objective.

Moreover, recent deepfake generation methods aim to preserve global facial structure and identity while minimizing perceptual artifacts, which further increases redundancy in non-critical regions. The discriminative evidence is therefore sparse relative to the full image, and storing entire facial images for replay retains large amounts of non-informative content. By compressing facial information and preserving only forgery-decisive regions, the replay strategy focuses on task-relevant evidence while discarding redundant identity-consistent signals. This selective retention reduces memory consumption and enables more diverse replay samples under a fixed storage budget, which is particularly beneficial for incremental deepfake detection.
\subsection{Replay Selection}
\subsubsection{Regional Density of Decisive Information.}
Firstly, we manage to expose the region in a single face that is the most decisive for the judgment of the detectors. At present, a variety of well-established techniques have been developed to obtain the decision-related attention regions of a model (either CNN-based~\cite{selvaraju2017gradcam,chattopadhay2018gradpp} or ViT-based~\cite{bousselham2025legrad,chefer2021transformergrad}) with respect to a given input image. Building upon these approaches, we incorporate forged information and propose to leverage the text-image alignment capacity of CLIP to highlight the forgery-related similarity of different patches. Specifically, given an input image $\mathbf{x}^{t-1} \in \mathbb{I}^{t-1}$, where $\mathbb{I}^{t-1}$ denotes the $t-1$ task, we can have a CLIP-based detector $f(\cdot,\theta^{t-1})$ with $t-1$ trained parameters $\theta^{t-1}$. We can then obtain a series of image tokens using $t-1$ encoder ($\mathit{E}(\cdot)$) as $\mathit{E}(\mathbf{x}^{t-1})=\{\mathbf{z}_{cls},\mathbf{z}_{(1,1)},...,\mathbf{z}_{(n,n)}\}$. Subsequently, to evaluate the forgery-decisive score ($\delta$) of each token, we compare the similarity of each token with the forgery-representative token ($\mathbf{z}_{f}$), which is obtained by encoding forgery-representative prompts via the text encoder. Since both text tokens and image tokens are pre-trained to be mapped to the consistent latent space, they can be directly leveraged to compare similarity. Formally, the forgery decisive score $\delta$ of the patch at location $(i,j)$ is calculated as:
\begin{equation}
    \delta_{(i,j)}=\text{Sim}(\mathbf{z}_{(i,j)},\mathbf{z}_{f}),
\end{equation}
where $\text{Sim}(\cdot)$ denotes computing cosine similarity.
Finally, we rank the patches based on their $\delta$ and filter out the top 10 patches as the Decisive Patches ($\mathbf{P}_\text{D}=\{\mathbf{p}_1,...,\mathbf{p}_{10}\}$) for each image. \\%我们基于分数对于不同pacth进行排序，并filter out top10的patch作为每张图中的Decisive patches.
\subsubsection{InfoDense Cut.} Here, we need to utilize the decisive patches $\mathbf{P}_\text{D}$ to guide the cutting extraction of the most info-dense partial region in each image. To achieve this, we first consider deploying ClockMix~\cite{cheng2025ed} as the cutting manner to extract regions that are dense in forgery information while maintaining semantic uniformity. Since ClockMix has already been proven to cut out segments in face forgery that evenly include identity, forgery, and background, we only need to focus on how to compute the ClockMix-segment that contains the maximum number of decisive patches in each image. Specifically, we employ a two-pointer scanning strategy. Given an angle ratio ofthe  extracted region ($n$) and two rays ($v_1$) and ($v_2$) with an angle of $\frac{360}n$, these two rays will scan all angles starting from the origin vertical one, ultimately obtaining the regional segment ($\mathbf{s}$) that contains the largest count of decisive patches as:
%With decisive attention, we then need to利用这些attention来截取每张图片中最适合回放用的infodense partial region。因此，我们想到了以clockmix作为手段，来得到forgery info 稠密，且语义均匀的区域。ClockMix已经被证明可以切出人脸伪造中，身份，伪造，和背景均匀包含的片段。因此，我们只需要考虑如何使用clockmix来切出每张图中包含decisive patch数量最大的区域。具体地说，我们采用了双指针扫描的遍历策略。给定一个region大小n（aka数据压缩比例 ）,以及对应的两条夹角固定为360/n的射线$v1,v2$, 这两条射线会从原点开始扫描所有角度，并最终记录包含的Decisive patch最多的InfoDense Segment as
\begin{equation}
    \mathbf{s}=\text{Cut}(\mathbf{x}) = \max_{\alpha \in [0, 360-360/n)} \left( \text{Count}_\text{D}(\text{Seg}(v_1,v_2,\alpha)) \right), 
\end{equation}
where $\text{Count}_\text{D}(\text{Seg})=\sum_{\mathbf{p} \in \mathbf{P}_\text{D}} \mathbf{I}\left( \mathbf{p}\text{\space within \space}\text{Seg}\right)$ represents the decisive patch count within the segment, $\mathbf{I}\left(\cdot\right)$ is an indicator that returns 1 when the input expression is true, $\alpha$ is the angle from begin to $v_1$. Based on the aforementioned algorithm, we can obtain the InfoDense Cut Segment set $\mathbf{S}=\{\mathbf{s},...\}$ corresponding to each image $\{\mathbf{x},...\} \in \mathbb{I}^{t-1}$.
%基于上述算法，我们可以得到$\mathbb{I}^{t-1}$中所有数据各自对应的InfoDense Cut Region集合$\mathbf{S}}$。
\\
\subsubsection{InfoDense Select.} Given a set of InfoDense Cut Segments, we further need to select the most information-dense one to be stored in the final replay buffer. Here, we consider both the latent-space centroid similarity~\cite{pan2023dfil} and the count of included decisive patches for the replay selection. This is because the central data of the distribution contains the most representative information of the overall dataset, while the decisive patch count represents the information that plays a critical role in forgery detection. Therefore, we combine the centroid distance and patch count with a weighted sum, which is then used for sorting. 
%一组InfoDense Cut Region,我们要进一步的选择信息丰富的块最终存入replay buffer。这里，我们同时考虑了segment的distribution centroid distance （cite DFIL）和 包含Decisive patch count来进行replay选取。这是因为分布的中心区域包含了最具数据集整体代表性的信息，而decisive patch count则代表了对于伪造判别起决定性作用的信息。具体地说，我们将中心距离和count进行了加权结合，以此作为排序的reference score。，即：
\begin{equation}
    \hat{\mathbf{S}} = \text{sort}\left(\mathbf{S},\cos(\mathbf{c},f(\mathbf{x}_i))+\text{Count}_\text{D}(\mathbf{s}_{i})\right),
\end{equation}
where $\mathbf{c} = |\mathbb{I}^{t-1}| \cdot \mathbb{E}[f(\mathbf{x})]$, $\mathbb{E}[\cdot]$ denotes the expectation operator.
Finally, we select the top-$m$ segments from $\hat{\mathbf{S}}$ and store them in the replay buffer as $\mathbf{S}^{t-1}$, where $m$ denotes the predefined replay set size.
%最后，我们在S中选取了前m个segment存入replay buffer S^{t-1}，其中m代表设定的replay set大小。
\subsection{Replay Utilization}
\subsubsection{InfoFuse.} Unlike conventional replay data that are intact and can be directly used for model training to prevent forgetting, InfoDense-replayed segments are actually fragmented data and cannot be directly fed into the model for training. Therefore, we consider fusing these fragmented InfoDense replays with the current-task data ($I^{t}$) to construct intact samples to facilitate model learning. That is, taking the current-task intact data as the foundations, and supplementing previous-task information by attaching InfoDense segments to them. Formally, given a replay segment ($\mathbf{s} \in \mathbf{S}^{t-1}$) and a current-task training sample ($\mathbf{x} \in \mathbb{I}^{t}$), the fusion can be written as:
%上述replay selection策略成功的得到了一组InfoDense Segment存入到了replay buffer。 however，不同于常规的replay数据是完整的，可以直接用于模型的训练以预防遗忘，InfoDense Segment实际上是不规则的数据形式，并不能直接送入模型中用于训练。因此，我们考虑将这些碎片化的infodense replay与$I^{t}$的数据进行fusion，以得到 形式规则的完整fusion图片数据用于训练。Formally, given segment $s \in S^{t-1}$ and current training sample $x \in I^t$, it can be written as:
\begin{equation}
    \mathbf{x}^t_\text{train}=\text{InfoFuse}(a, b) = \max(\mathbf{x}, \mathbf{s} \cdot \mathbb{I}_{\mathbf{s} = 0}), \label{eq:fuse}
\end{equation}
where $\max(\cdot)$ is selecting the larger values at each pixel, $\mathbb{I}_{\mathbf{s} = 0}=0$ if $\mathbf{s} = 0$. \\%上述过程可以被相同的应用于更之前的replay segment上。
\subsubsection{Multi-Fused Samples.}
Due to the various existence of current task data, past task data, and the combinations of their real/fake labels, the strategy behind their pairings and the labeling requires further analysis. We adopt the labeling strategy among real/fake combinations from ClockMix~\cite{ED4}, where any inclusion of ``fake'' segment is labeled as fake. This is because we want to ensure that all real/fake data in the replay buffer is effectively utilized for real/fake judgment training. Then, the combinations among previous and current tasks are newly introduced by our mixing paradigm and need to be carefully designed here. For simplicity, we use (t-1) to represent all past task data.\\
1. \textbf{(t) \& (t-1) inter-task}: We perform a full combination of the real/fake labels from (t-1) and (t) (i.e., $2\times2=4$ combinations). By mixing data with different labels for replay, we impose a constraint that helps the model learn the full information in the replay buffer and prevents class bias.\\
2. \textbf{(t) intra-task}: To ensure that the model maintains desensitization with fused images that contain junctions, we also perform random mixing of real/fake labels within the (t) task. This prevents the model from generating erroneous spurious mappings—i.e., images with fusion are incorrectly assumed to belong to (t-1) task, which could introduce task bias in the model's learned information.\\
3. \textbf{Multi-Seg}: Past (t-1) segments can be fused with multiple instances of the (t) task based on Eq.~\ref{eq:fuse}, increasing the information content from the past task and enhancing the influence of past samples during supervised training, thereby reducing forgetting. Moreover, multi-segment fusion can further enhance data diversity and the granularity of subtle forgery clues.

All of the aforementioned types of fused samples, along with the original images from the (t)-task, form a mini-batch for training the (t)-task model ($f(\cdot, \theta^t)$).
In summary, Multi-Fused samples have the following three advantages:
1. They allow fragmented regional replay data to be effectively utilized in an intact form for replay training.
2. The fusion strategy prevents class and task biases that could arise from the introduction of fusion among different tasks and labels.
3. Fused samples contain more diverse and fine-grained information, enhancing the model's ability to learn generalizable and subtle knowledge.


%由于存在当前task数据，过往task数据，以及真假等多种组合情况，其两两搭配的合理性与label的分配策略需要进一步的分析。 为了方便叙述，我们用t-1来代表所有过往任务的数据。（1）t\&(t-1) inter-task：这里，我们将t-1的real/fake与t的real/fake进行了全量的组合（即包含2x2=4种），并沿用cite中的包含fake即是fake的labeling策略。这是因为我们希望确保replay buffer中的所有real/fake都被有效利用，而通过不同label对于不同回放数据的混合约束，可以帮助模型更好的学习replay中的全量信息，防止class bias。（2）t intra-task：为了使模型维持对于带有fusion接缝图片的脱敏，我们也同时对t task内部的真伪进行了随机的混合，进而防止模型产生错误的suprious映射：即包含fusion的图片就被认为是t-1 task，导致模型学习的信息产生task bias。（3）Multi-Seg: 过往的t-1 segment 可以被多个fusion到t task上，使得过往task的信息含量上升，提高监督训练时过往样本的影响，降低遗忘率。Moreover，multi-seg fusion可以进一步的提高数据的多样性。上述的所有类型fused 样本将与t-task的原图一起组成mini-batch，对t-task 的模型f(,\theta^t)进行训练。

%综合来说，Multi-Fused samples 有如下四个优点：1）使不规则的regional 回放数据被以规则的形式有效用于回放训练。2）通过fusion的组合策略， 我们防止了由于引入fusion而导致的class and task bias。3）单张样本包含更diverse的信息，提高了模型学习到通用泛化信息的能力、

==> icml/sec/doc/intro.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{sec/fig/intro.pdf}
    \caption{}
    \label{fig:intro}
\end{figure}
\section{Introduction}
The rapid advancement of generative technologies has led to increasingly diverse and realistic forgery faces, posing serious threats to multimedia security and social trust. One line of research seeks to address this challenge by training forgery detection models with strong generalization ability under limited data conditions, so as to improve robustness to unseen forgeries. However, generalization-oriented approaches \cite{sun2022dual,cao2022end,huang2023implicit,yan2024transcending,cheng2024can,cheng2025ed} can only partially handle unknown forgery patterns and still struggle to cope with the continuous evolution of forgery techniques. To this end, incremental forgery detection has recently attracted growing attention, aiming to progressively learn new forgery types while maintaining reliable detection performance on previously learned ones.

Incremental forgery detection methods typically mitigate catastrophic forgetting by replaying representative samples during the learning of new data. Common strategies include central sample replay \cite{pan2023dfil}, hard sample replay \cite{pan2023dfil}, adversarial perturbation–based replay \cite{sun2025continual}, mixed prototypes \cite{tian2024dynamic}, and sparse uniform replay \cite{cheng2025stacking}. However, these replay-based approaches inevitably require storing raw historical samples, resulting in non-negligible memory overhead and potential privacy risks. Notably, face images exhibit strong structural regularities, such as bilateral symmetry and the spatial concentration of discriminative cues. For deepfake detection, the information required for effective replay mainly concerns identity-related features, forgery artifacts, and domain-specific patterns. These cues are typically localized and redundantly distributed across symmetric facial regions, rather than being uniformly spread over the entire face. Consequently, storing the full face image is not strictly necessary to preserve replay knowledge. Selectively retaining informative facial regions can sufficiently maintain the critical information needed to alleviate forgetting in incremental deepfake detection.

Motivated by the above observations, we aim to design a regional decisive replay strategy that preserves essential forgery knowledge while significantly reducing storage cost. As illustrated in Fig. 1, we attempt to model and visualize the decisive attention of samples during detector training. Based on the resulting attention distribution, forgery face images can be conceptually divided into information-dense regions and information-sparse regions. The former captures critical domain characteristics and forgery traces, while the latter mainly contain redundant information. During replay, we preferentially retain the information-dense facial regions, which enables effective knowledge preservation while substantially reducing the memory cost required for replay. In this way, more historical samples can be replayed under the same storage budget, effectively alleviating catastrophic forgetting. Moreover, by replaying compact regions that concentrate essential forgery cues, the detector is encouraged to focus on the core factors underlying forgery, which further enhances its generalization to unseen manipulations.


\section{Related Works}
\subsection{Face Forgery Detection}
Existing generalization-oriented face forgery detection methods typically leverage a limited set of known forged samples to train a generic detector capable of handling unseen forgery types. Early studies primarily enhance discriminative capability by exploiting explicit forgery-related patterns, such as noise artifacts \cite{li2020face}, local region cues \cite{chen2021local,zhao2021multi}, and frequency-domain information \cite{qian2020thinking,guo2020learning,kashiani2025freqdebias}. As forgery techniques become increasingly realistic, explicit artifacts tend to diminish, shifting research focus toward mining implicit forgery patterns. To this end, a variety of learning strategies have been proposed, including contrastive learning \cite{sun2022dual}, identity-aware modeling \cite{huang2023implicit,dong2023implicit}, disentangled representation learning \cite{liang2022exploring,yan2023ucf}, reconstruction-based learning \cite{cao2022end,wang2021representative}, and diverse data augmentation techniques \cite{chen2022self,shiohara2022detecting,yan2024transcending}. More recently, several approaches based on vision Transformers have leveraged vision–language models, such as CLIP \cite{cui2025forensics} and the LoRA-based Effort \cite{yan2025effort}, to further enhance generalization performance. Overall, existing approaches strive to derive forgery-aware representations that generalize beyond known manipulations. Yet, due to the limited coverage of current forgery datasets, detectors trained under a static offline setting struggle to remain effective when confronted with continuously emerging forgery techniques.
\subsection{Incremental Learning for Forgery Detection}
Incremental learning has been widely applied to mitigate catastrophic forgetting, with replay-based strategies dominating the face forgery detection domain. These methods store or reuse representative samples from previous tasks and employ various enhancements to preserve prior knowledge. For instance, CoReD \cite{kim2021cored} uses knowledge distillation to retain information from past tasks. DFIL \cite{pan2023dfil} prioritizes central and challenging samples to maximize the value of replayed data. HDP \cite{sun2025continual} leverages carefully crafted universal adversarial perturbations for more robust rehearsal. DMP \cite{tian2024dynamic} summarizes previous distributions through mixed prototypes. The most recent method, SUR-LID \cite{cheng2025stacking}, combines sparse uniform replay with a latent-space incremental detector to further consolidate prior knowledge. While effective, all of these approaches rely on explicit access to stored historical data, which imposes non-negligible memory overhead and raises potential privacy concerns.

In continual learning, several studies have explored compressed replay to reduce storage cost and store more historical samples under a fixed memory budget, such as compressing exemplars by removing non-discriminative pixels \cite{luo2023class} or selecting an appropriate compression quality for replay \cite{wang2022memory}. However, existing compressed replay methods are largely developed for generic class-incremental settings and typically operate at the image or pixel level, without explicitly considering the task-specific structure of face forgery detection. In this domain, replay is expected to preserve identity cues, forgery traces, and domain-specific patterns that may exhibit distinct spatial distributions, suggesting that more tailored replay compression strategies still remain to be explored.


==> icml/sec/doc/method.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{sec/fig/pipeline.pdf}
    \caption{}
    \label{fig:pipeline}
\end{figure*}
\section{Proposed Method}
To compress the redundant information in the facial data, thus improving the diversity and info-density within the same storage consumption, we propose a unified framework termed InfoDense that can  select, and utilize the data region with dense information for replay. The overall pipeline can be found in Fig.~\ref{fig:pipeline}.
\subsection{Rational Behind Compressing Facial Information}
% 师兄帮忙写一下
\subsection{Replay Selection}
\textbf{Regional Density of Decisive Information.}\\
Firstly, we manage to expose the region in single face that decides the judgment of the detectors. To achieve this goal, we consider leveraging the text-image alignment capacity of CLIP to highlight the forgery-related similarity of different patches. Specifically, given an input image $\mathbf{X}^{t-1} \in \mathbb{I}^{t-1}$, where $\mathbb{I}^{t-1}$ denotes the $t-1$ task, we can have a CLIP-based detector $f(\cdot,\theta^{t-1})$ with $t-1$ trained parameters $\theta^{t-1}$. We can then obtain a series of image tokens using $t-1$ encoder ($\mathit{E}(\cdot)$) as $\mathit{E}(\mathbf{X}^{t-1})=\{\mathbf{z}_{cls},\mathbf{z}_{(1,1)},...,\mathbf{z}_{(n,n)}\}$. Subsequently, to evaluate the forgery-decisive score ($\text{s}_{fd}$) of each token, we compare the similarity of each token with the forgery-representative token ($\mathbf{z}_{f}$), which is obtained by encoding forgery-representative prompts via the text encoder. Formally, the $text{s}_{fd}$ of each patch is calcualted as:
\begin{equation}
    \text{s}_{fd}=
\end{equation}
Finally, we rank the patches based on their $\text{s}_{fd}$ and filter out the top 10 patches as the Decisive patches for each image.%我们基于分数对于不同pacth进行排序，并filter out top10的patch作为每张图中的Decisive patches.
\textbf{InfoDense Cut}\\
\textbf{InfoDense Select}
\subsection{Replay Utilization}
\textbf{InfoFuse}\\
\textbf{Fusion Strategy}
